QUBIC II: Spectro-Polarimetry with Bolometric Interferometry

Bolometric interferometry is a novel technique that has the ability to perform spectral imaging. A bolometric interferometer observes the sky in a wide frequency band and can reconstruct sky maps in several sub-bands within the physical band in post-processing of the data. This provides a powerful spectral method to discriminate between the cosmic microwave background (CMB) and astrophysical foregrounds. In this paper, the methodology is illustrated with examples based on the Q \& U Bolometric Interferometer for Cosmology (QUBIC) which is a ground-based instrument designed to measure the B-mode polarization of the sky at millimeter wavelengths. We consider the specific cases of point source reconstruction and Galactic dust mapping and we characterize the point spread function as a function of frequency. We study the noise properties of spectral imaging, especially the correlations between sub-bands, using end-to-end simulations together with a fast noise simulator. We conclude showing that spectral imaging performance are nearly optimal up to five sub-bands in the case of QUBIC.

==> correction_section3-2 <==
%--------------------------------------------------
\subsection{Spectral imaging capabilities}\label{ss:SI-capabilities}
The synthesized beam at two different frequencies $\nu_1$ and $\nu_2$ will be distinguishable from one another as long as their peaks are sufficiently separated.
The angular separation between the two peaks $\Delta \theta= \frac{c \Delta \nu}{\nu^2 \Delta h}$ (where $\Delta\nu=\nu_2-\nu_1$ and $\nu=\sqrt{\nu_1\nu_2}$) must be large enough to unambiguously distinguish the two peaks. In order to have an order of magnitude of the possible width for each sub-band we consider a square array of pupils and we apply the Rayleigh criterion~\cite{rayleigh1879xxxi}:  
\begin{eqnarray}
    \frac{c \Delta \nu}{\nu^2 \Delta h} \gtrsim \frac{c}{\nu(P-1)\Delta h} 
    \quad \Leftrightarrow \quad 
    \Delta\nu \gtrsim \frac{\nu}{(P-1)}
\label{eq:Rayleigh_criteria}
\end{eqnarray}
where $P$ is the number of pupils on a side of the square-packed pupil-array. A bolometric interferometer therefore not only has a resolution on the sky $\mathrm{FWHM}_\theta \simeq \frac{c}{\nu (P-1) \Delta h}$, but also in electromagnetic frequency space $\frac{\Delta\nu}{\nu}\simeq\frac{1}{P-1}$. 

The map-making presented in section~\ref{ss:mapmaking} can be extended in order to build, simultaneously, with the same TOD, maps at a number of different frequencies as long as they comply with the frequency separation given above. The iterative TOD $\vec{y_i}$ can be written as:
\begin{equation}\label{eqmmfreq}
    \vec{y_i} = \sum_{j=0}^{N_{\rm rec}-1} H_j \hat{\vec{s}}_{ij} + \vec{n}
\end{equation}
where $H_j$ describes the acquisition (convolution$+$pointing) operator with the synthesized beam at frequency $\nu_j$, $\hat{\vec{s}}_{ij}$ is the sky signal estimator at iteration $i$ for the frequency $\nu_j$ and $N_{\rm rec}$ is the number of reconstructed sub-bands. Similarly, as in the map at a single frequency (figure~\ref{fig:fig_mm}), one can recover the maps $\vec{s_j}$ by solving equation~(\ref{eqmmfreq}) using a preconditioned conjugate-gradient method (see section~\ref{sec:testSection} for corresponding simulations). Thus, the instrument acquires data in a single wide frequency band and spectral imaging technique applies during map-making, in the post-processing of the data.

The QUBIC FI has two wide-bands centered at 150 and 220~GHz with $\Delta\nu/\nu=0.25$
and a 400-feedhorn array
packed on a square grid within a circular area (see figure~\ref{fig:fig_beamFP}). We approximate it with a square grid $20\times 20$ so $\frac{1}{(P-1)}\sim 0.05$. It is thus possible to reconstruct approximately 5~sub-bands in each of the initial bands of QUBIC. Note that this number should just be taken as an order of magnitude for the achievable number of sub-bands but we will see in figure~\ref{fig:resolutions} that it is a good approximation. In section~\ref{sec:noiseSection} we will show that reconstructing up to 8 sub-bands is feasible but with a significant degradation of the signal-to-noise ratio.

